Large Language Model-Driven Dynamic Assessment of Grammatical Accuracy in English Language Learner Writing

This study investigates the potential for Large Language Models (LLMs) to scale-up Dynamic Assessment (DA). To facilitate such an investigation, we first developed DynaWrite-a modular, microservices-based grammatical tutoring application which supports multiple LLMs to generate dynamic feedback to learners of English. Initial testing of 21 LLMs, revealed GPT-4o and neural chat to have the most potential to scale-up DA in the language learning classroom. Further testing of these two candidates found both models performed similarly in their ability to accurately identify grammatical errors in user sentences. However, GPT-4o consistently outperformed neural chat in the quality of its DA by generating clear, consistent, and progressively explicit hints. Real-time responsiveness and system stability were also confirmed through detailed performance testing, with GPT-4o exhibiting sufficient speed and stability. This study shows that LLMs can be used to scale-up dynamic assessment and thus enable dynamic assessment to be delivered to larger groups than possible in traditional teacher-learner settings.

==> methods.tex <==
\section{Methods}

\subsection{Overview and Objectives}
We developed the web application \textbf{Dynawrite} to address two main tasks: improving English language learning through interactive grammar checking and providing a platform for evaluating NLP models in real-world educational settings.
The application is designed to assist users in writing texts and providing feedback, with a particular focus on those for whom English is not their native language but who use it to communicate in a digital environment.
 
The Dynawrite project is driven by three primary objectives: enhancing learning outcomes, advancing NLP model evaluation, and ensuring modularity and scalability.
Designed as a pedagogically grounded tool, Dynawrite helps English language learners correct grammatical errors step by step while providing detailed and constructive recommendations to improve their skills.
It offers researchers robust tools to analyze various NLP models' performance, efficiency, and precision in real-world writing tasks.
Additionally, its scalable architecture allows for the seamless addition or replacement of NLP models, minimizing the need for extensive reconfiguration and ensuring adaptability for future developments.

The system serves two key user groups.
For students and teachers, Dynawrite simplifies the English language learning process through an intuitive interface that leverages NLP models to provide step-by-step corrections for grammatical errors.
For researchers and developers, the platform offers a detailed framework to evaluate NLP models, assessing parameters such as response time, accuracy in error detection, and the quality of feedback provided.

Among Dynawrite's standout features is its hierarchical hint system, which guides users through correcting errors.
The system begins with subtle suggestions and gradually provides more explicit instructions until the correct solution is understood.
This structured feedback mechanism enhances the learning experience and fosters a deeper understanding of grammatical concepts.
The system's microservices-based architecture, powered by Apache Kafka, supports dynamic model integration, enabling users to seamlessly add, remove, or replace NLP models without disrupting the workflow.
This flexibility ensures that Dynawrite remains a cutting-edge tool for education and research.


\subsection{System Architecture}
The Dynawrite system uses a modular microservices architecture, making it scalable, reliable, and easy to integrate (Figure~\ref{fig:architecture}).
The diagram shows how users interact with different parts of the system.
Users work through a VueJS-powered front-end, serviced using Nginx, which connects to a Go/Gin-based REST API backend.
The Apache Kafka message broker facilitates communication between microservices responsible for NLP models, reporting, and real-time updates.
Each system component supports flexibility and scalability.
The architecture uses PostgreSQL for data storage and Keycloak for authentication.
Separate microservices connect NLP models like GPT-4o-mini and Llama3.2.
The system consists of six microservices, each with a distinct task.
Additional infrastructure components ensure the system's stable and efficient operation.

\begin{figure*}[h!]
  \centering
  \includegraphics[width=\textwidth]{methods/architecture.png}
  \Description{The architecture of the Dynawrite system, showcasing its modular and scalable microservices-based design.}
  \caption[System Architecture]{The architecture of the Dynawrite system.}
  \label{fig:architecture}
\end{figure*}

The six microservices in Dynawrite are summarized in Table~\ref{tab:microservices}, along with their respective roles.

\begin{table}
\caption{Microservices in Dynawrite}
\label{tab:microservices}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{|p{85pt}|p{140pt}|}
\hline
\textbf{Microservice} & \textbf{Description} \\ \hline
REST API & Provides core backend functionality for processing user requests, authenticating users, and managing interaction with Apache Kafka.\\ \hline
Dynawrite\_Consumer & Listens to Apache Kafka messages, processes NLP responses, stores results in PostgreSQL, and sends updates to Centrifugo.\\ \hline
Ollama\_Consumer & Handles requests for NLP models in the Ollama framework, such as Llama3 and Gemini.\\ \hline
OpenAI\_Consumer & Manages communication with the OpenAI ChatGPT API for text analysis.\\ \hline
Export\_Consumer & Generates reports in Excel and CSV formats, detailing NLP model performance and user interaction data.\\ \hline
CPush\_Consumer & Sends real-time updates to the frontend via WebSocket channels.\\ \hline
\end{tabular}
\end{table}


\subsubsection{Supporting Infrastructure}
The architecture also includes the following infrastructural components:
\begin{itemize}
    \item \textbf{Nginx}: Served as a reverse proxy for the VueJS frontend and Go backend.
    \item \textbf{Apache Kafka}: Facilitates asynchronous communication between microservices through well-defined topics (Table~\ref{tab:kafka_topics}).
    \item \textbf{PostgreSQL}: Stores user data, session logs, and NLP analytics in a relational schema.
    \item \textbf{VueJS}: Implements the user interface, which is compiled into static files served by Nginx.
    \item \textbf{Centrifugo}: Ensures responsive, real-time feedback for users interacting with the system.
    \item \textbf{Keycloak}: Manages user authentication and role-based access control.
\end{itemize}

\begin{table}
\caption{Kafka Topics Used in Dynawrite}
\label{tab:kafka_topics}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{|p{75pt}|p{150pt}|}
\hline
\textbf{Topic Name} & \textbf{Purpose} \\ \hline
nlp\_request\_text & Sends text analysis requests to NLP microservices.\\ \hline
nlp\_response\_text & Receives error analysis and correction hints from NLP models.\\ \hline
cent\_push\_message & Delivers real-time feedback to the frontend.\\ \hline
reports\_export\_topic & Handles requests for generating analytical reports.\\ \hline
\end{tabular}
\end{table}

\subsection{Functionalities}

The Dynawrite system provides a comprehensive set of functionalities designed to cater to three primary user groups: students, teachers, and researchers.
Each group benefits from tailored tools and features aimed at enhancing the user experience, improving learning outcomes, and supporting research.

\subsubsection{Student Functionalities}

Students are the primary end-users of the system, utilizing Dynawrite as a learning platform to improve their English language skills.
Key functionalities include:

\paragraph{Workbook for Text Correction}
\begin{itemize}
    \item Students can create text documents in the \textbf{Workbook} section (Figure~\ref{fig:workbook_screenshot}).
    \item The system processes the text sentence by sentence, analyzing it for grammatical errors using selected NLP models.
    \item Feedback is provided through a \textbf{hierarchical hint system}, offering four levels of detail:
    \begin{enumerate}
        \item \textbf{Level 1: Implicit Hint}: Indicates the presence of an error without specifying details.
        \item \textbf{Level 2: Contextual Clue}: Highlights the part of the sentence likely containing the error.
        \item \textbf{Level 3: Metalinguistic Explanation}: Provides a linguistic explanation of the error (e.g., noun-verb agreement).
        \item \textbf{Level 4: Explicit Correction}: Suggests the correct version of the sentence.
    \end{enumerate}
    \item Students can attempt corrections up to four times per sentence, progressively receiving more detailed hints if errors persist.
    \item Sentences corrected successfully are marked as \textbf{“completed”}, while uncorrected sentences are logged for further review.
\end{itemize}

\begin{figure*}[h!]
  \centering
  \includegraphics[width=\textwidth]{methods/screenshot.png}
  \Description{The Dynawrite Workbook interface, displaying a student's session
  The interface shows the analyzed sentence with a hierarchical hint for correction, allowing students to progressively improve their sentence until it is grammatically correct.}
  \caption[Dynawrite Workbook Interface]{The Dynawrite Workbook interface.
  This screenshot illustrates a student working on sentence corrections, receiving a Level 2 hint highlighting a potential issue in the sentence.
  Key parameters like the NLP model, temperature, and token settings are displayed for transparency.}
  \label{fig:workbook_screenshot}
\end{figure*}

\paragraph{Progress Tracking}
\begin{itemize}
    \item Students can view a history of their previous sessions, including:
    \begin{itemize}
        \item The number of errors identified and corrected.
        \item The level of hint required to correct each sentence.
        \item A summary of uncorrected sentences.
    \end{itemize}
    \item Visual progress indicators, such as graphs or percentages, help students track their improvement over time.
\end{itemize}

\paragraph{Real-Time Feedback}
\begin{itemize}
    \item Real-time error analysis is powered by NLP models and delivered to students through the Centrifugo-based WebSocket system.
    \item Instant feedback enhances the learning experience by maintaining engagement and minimizing delays.
\end{itemize}

\subsubsection{Teacher Functionalities}

Teachers play a crucial role in guiding students and monitoring their progress.
Dynawrite provides educators with the following tools:

\paragraph{Course and Task Management}
\begin{itemize}
    \item Teachers can create and assign courses consisting of multiple tasks, including:
    \begin{itemize}
        \item \textbf{Image Description Tasks}: Students describe an image in English based on a given prompt.
        \item \textbf{Text Correction Tasks}: Students correct pre-defined sentences containing intentional errors.
    \end{itemize}
    \item Tasks are customizable with parameters such as:
    \begin{itemize}
        \item Specific NLP models for text analysis.
        \item Difficulty level and error types for text correction tasks.
        \item Additional guidelines for students.
    \end{itemize}
\end{itemize}

\paragraph{Monitoring Student Performance}
\begin{itemize}
    \item Teachers can access detailed reports on student performance, including:
    \begin{itemize}
        \item Success rates for text corrections.
        \item The average number of attempts required per sentence.
        \item Hints utilized at each level of detail.
    \end{itemize}
    \item Aggregate metrics are presented visually, allowing teachers to identify common areas of difficulty among students.
\end{itemize}

\paragraph{Report Generation}
\begin{itemize}
    \item Teachers can generate downloadable reports in CSV and Excel for further analysis.
    \item Reports include details such as:
    \begin{itemize}
        \item The NLP model used for analysis.
        \item Response times and accuracy metrics.
        \item Sentence-level summaries of student performance.
    \end{itemize}
    \item These reports are particularly useful for identifying patterns and tailoring future assignments to address specific challenges.
\end{itemize}

\subsubsection{Researcher Functionalities}

The Dynawrite system is designed with modularity and advanced analytics, making it a valuable resource for researchers investigating the performance of NLP models in educational settings.
Its architecture allows for detailed evaluation, benchmarking, and data collection to support cutting-edge research.


One of the system’s key features is its capability for comparative analysis of NLP models.
Researchers can evaluate multiple models based on metrics such as average response time, standard deviation, percentiles, accuracy in detecting grammatical errors, and the rates of false positives and negatives.
The system provides visual insights through detailed graphs and charts (e.g., Figures~\ref{fig:avg_response_time}–\ref{fig:accuracy}), which enable a comprehensive understanding of model performance.


In addition to comparative analysis, Dynawrite supports performance benchmarking by allowing researchers to integrate new NLP models via Apache Kafka.
The system automatically collects and stores performance metrics, creating a structured dataset for in-depth evaluation and optimization of these models.


Another significant feature is its capability for dataset collection and annotation.
The system logs anonymized user interactions, including data on error correction attempts and the effectiveness of hierarchical hints.
These datasets are instrumental in training and fine-tuning future NLP models and are valuable for conducting broader linguistic research and understanding user behavior.


By combining these functionalities, Dynawrite offers researchers a powerful platform to explore the potential of NLP models and contribute to advancements in educational technology and computational linguistics. 


\subsubsection{Cross-Group Functionalities}

Some functionalities are shared across all user groups, enhancing the overall experience:
\begin{itemize}
    \item \textbf{User Authentication and Role Management}: Managed through Keycloak, ensuring secure access based on user roles (student, teacher, or researcher).
    \item \textbf{Real-Time Updates}: Powered by Centrifugo, ensuring instant feedback and seamless interaction between users and the system.
    \item \textbf{Accessibility}: The system’s responsive design ensures compatibility with various devices, including desktops, tablets, and smartphones.
\end{itemize}

\subsection{Development Process}

The development of Dynawrite followed an iterative, structured approach, ensuring modularity, scalability, and adaptability to future advancements in NLP technologies.
This section outlines the key stages and methodologies employed during the project lifecycle.

\subsubsection{Requirements Analysis and Initial Prototyping}
The project began with a thorough requirements analysis to identify the primary objectives:
\begin{itemize}
    \item To support multiple NLP models for text analysis and error correction.
    \item To provide a flexible framework capable of integrating emerging NLP technologies.
    \item To design a user-friendly interface for students and educators.
\end{itemize}

An initial prototype was developed in Python, using the OpenAI ChatGPT API for text analysis.
This prototype focused on:
\begin{itemize}
    \item Sentence-by-sentence grammar checking.
    \item Generating multi-level hints for error correction.
    \item Collecting feedback from early users (students and teachers) to refine functionalities.
\end{itemize}
This stage helped validate the core concept and identify potential technical challenges, such as the need for real-time processing and support for multiple NLP models.

\subsubsection{Transition to Microservices Architecture}
The system was redesigned using a microservices-based architecture to meet the scalability and modularity requirements.
The transition involved:
\begin{enumerate}
    \item Rewriting the backend from Python to Go, leveraging the GIN framework for efficient REST API development.
    \item Designing a Kafka-based message broker to decouple services, ensuring seamless communication between components.
    \item Developing independent microservices for specific tasks, such as:
    \begin{itemize}
        \item NLP model integration (\texttt{ollama\_consumer}, \texttt{openai\_consumer}).
        \item Real-time updates (\texttt{cpush\_consumer}).
        \item Report generation (\texttt{export\_consumer}).
    \end{itemize}
\end{enumerate}

This architecture enabled the system to dynamically integrate and replace NLP models without affecting the core functionalities.

\subsubsection{Frontend Development}
The frontend was implemented using VueJS, and designed for responsiveness and compatibility with various devices.
Key features included:
\begin{itemize}
    \item A dashboard for students to manage assignments and track progress.
    \item A course creation interface for teachers to design and assign tasks.
    \item Real-time feedback display, supported by Centrifugo for WebSocket-based communication.
\end{itemize}

The VueJS application was bundled into static files and served via Nginx, ensuring high performance and minimal latency for end users.

\subsubsection{Integration of NLP Models}
One of the critical aspects of development was integrating and testing multiple NLP models.
This involved:
\begin{itemize}
    \item Implementing the \texttt{ollama\_consumer} microservice to process requests for models such as \texttt{Llama3.2} and \texttt{Vicuna}.
    \item Developing the \texttt{openai\_consumer} microservice for handling requests to the OpenAI ChatGPT API.
    \item Designing a unified interface for sending and receiving data from models, ensuring consistent feedback formatting.
    \item Benchmarking models based on response time, accuracy, and computational requirements (as detailed in Figures~\ref{fig:avg_response_time}–\ref{fig:percentiles}).
\end{itemize}

\subsubsection{Report Generation and Analytics}
The report generation functionality was implemented to enable educators and researchers to:
\begin{itemize}
    \item Export detailed analysis of text corrections in Excel and CSV formats.
    \item Compare performance metrics of different NLP models.
    \item Visualize trends in student performance and model accuracy over time.
\end{itemize}

The \texttt{export\_consumer} microservice handled report creation, leveraging PostgreSQL for data storage and retrieval.

\subsubsection{Iterative Testing and Optimization}
Testing was conducted iteratively throughout development, focusing on:
\begin{enumerate}
    \item Unit testing of individual microservices to ensure robustness.
    \item Integration testing to validate seamless communication between components.
    \item Performance testing to identify bottlenecks and optimize response times.
    \item User feedback to refine the UI and improve the hint generation logic.
\end{enumerate}

Optimization efforts included:
\begin{itemize}
    \item Reducing the response time for NLP models by fine-tuning request payloads.
    \item Implementing caching mechanisms for frequently used data.
    \item Enhancing database queries to minimize latency.
\end{itemize}

\subsubsection{Deployment and Infrastructure Setup}
The system was deployed on a VPS with the following specifications:
\begin{itemize}
    \item 8 GB RAM, 6 CPUs, 100 GB SSD storage, suitable for hosting the core microservices and frontend/backend components.
    \item A MacBook Pro 14 (Apple M2 Pro, 16GB) was utilized for running Ollama models offline, ensuring local processing capabilities for resource-intensive NLP tasks.
    \item Support for Docker-based containerization to streamline the deployment of microservices.
\end{itemize}

\subsubsection{Task Management and Collaboration}
Task management was conducted using Trello with a Kanban methodology.
Key practices included:
\begin{itemize}
    \item Breaking down features into manageable tasks.
    \item Prioritizing tasks based on user feedback and system requirements.
    \item Conducting weekly meetings with collaborators to review progress and address challenges.
\end{itemize}

Collaboration tools such as Slack were used for real-time communication, while Codeberg served as the version control system for managing code repositories.

\subsubsection{Challenges and Solutions}
Several challenges were encountered during development:
\begin{itemize}
    \item \textbf{Challenge}: Handling variability in NLP model response times.
          \newline \textbf{Solution}: Implementing asynchronous request handling via Apache Kafka and optimizing payload structures.
    \item \textbf{Challenge}: Integrating multiple NLP models with differing APIs.
          \newline \textbf{Solution}: Designing a unified interface for model communication, abstracting differences in API structures.
    \item \textbf{Challenge}: Balancing performance with resource constraints on the VPS.
          \newline \textbf{Solution}: Utilizing lightweight microservices and optimizing database queries to reduce computational overhead.
\end{itemize}

\subsubsection{Future Development Plans}
Future iterations of the system will focus on:
\begin{itemize}
    \item Enhancing scalability by migrating to Kubernetes for container orchestration.
    \item Expanding the range of supported NLP models, including models specialized for low-resource languages.
    \item Adding offline capabilities for mobile and edge devices to increase accessibility.
\end{itemize}

\subsection{Testing and Analytics}

Testing and analytics were critical to evaluating the performance, accuracy, and efficiency of the Dynawrite system.
This section outlines the methodologies employed during testing, the insights derived from analytics, and how these results shaped system improvements.

\subsubsection{Testing Methodologies}
The following testing methodologies were employed to ensure the reliability and functionality of the system:

\paragraph{Unit Testing}
Each microservice was tested individually to verify its correctness and robustness.
Particular attention was given to:
\begin{itemize}
    \item Processing Kafka messages for both valid and invalid inputs.
    \item Handling database interactions in PostgreSQL.
    \item Ensuring compatibility with multiple NLP models.
\end{itemize}

\paragraph{Performance Testing}
Performance testing focused on analyzing:
\begin{itemize}
    \item \textbf{Average Response Time}: The time taken by each model to process a request.
    Figure~\ref{fig:avg_response_time} presents the average response times of tested models.
    \item \textbf{Response Time Stability}: Standard deviation of response times for each model, depicted in Figure~\ref{fig:response_stability}.
    \item \textbf{Scalability}: The ability to handle concurrent user requests without significant performance degradation.
\end{itemize}

\paragraph{Accuracy Testing}
The accuracy of NLP models was evaluated using:
\begin{itemize}
    \item \textbf{False Positive and Negative Rates}: The rates at which models incorrectly identified errors (false positives) or failed to detect errors (false negatives).
    Results are shown in Figure~\ref{fig:false_rates}.
    \item \textbf{Overall Accuracy}: The percentage of correct error detections, visualized in Figure~\ref{fig:accuracy}.
\end{itemize}

\paragraph{User Feedback and Usability Testing}
Feedback from students, teachers, and researchers was collected during User Acceptance Testing (UAT).
Suggestions included:
\begin{itemize}
    \item Improving the user interface for non-technical users.
    \item Enhancing the clarity of generated hints.
    \item Streamlining the process for generating reports.
\end{itemize}

\subsubsection{Analytics and Insights}

Comprehensive analytics were conducted to evaluate both user behavior and the performance of NLP models within the system.
User interaction data provided valuable insights into the learning process, capturing metrics such as the average number of attempts required to correct a sentence and the effectiveness of the hierarchical hint system in guiding users toward accurate corrections.
Additionally, longitudinal tracking allowed for an analysis of user progress over multiple sessions, shedding light on the system’s impact on learning outcomes.

Visualized insights further enhance the understanding of model performance.
Figures~\ref{fig:avg_response_time} through \ref{fig:percentiles} summarize key metrics, offering a clear comparison across models:
\begin{itemize}
	\item Figure~\ref{fig:avg_response_time}  illustrates the average response time for each model, highlighting overall efficiency.
	\item Figure~\ref{fig:response_stability} showcases the standard deviation of response times, providing a measure of stability in model performance.
	\item Figure~\ref{fig:false_rates} details the false positive and false negative rates, emphasizing the reliability of error detection.
	\item Figure~\ref{fig:accuracy} presents the accuracy of grammatical error detection, demonstrating each model’s effectiveness.
	\item Figure~\ref{fig:percentiles} outlines response time percentiles (25th, 50th, 75th), offering a nuanced view of model responsiveness under varying conditions.
\end{itemize}
These analytics and visual summaries provide a comprehensive understanding of both user engagement and the technical performance of the integrated NLP models, serving as a foundation for further optimization and research.

\subsubsection{Ollama Model Details}
The models used during testing are summarized in Table~\ref{tab:ollama_models_sorted}.
Their sizes and descriptions provide insights into their computational requirements and capabilities.

\begin{table}
\caption{Summary of Ollama Models Used in Testing (Sorted by Size)}
\label{tab:ollama_models_sorted}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{|p{75pt}|p{25pt}|p{115pt}|}
\hline
\textbf{Model Name} & \textbf{Size (GB)} & \textbf{Description} \\ \hline
\texttt{gemma2} & 5.4 & An advanced model developed for handling complex linguistic tasks with high proficiency.\\ \hline
\texttt{aya-expanse} & 5.1 & A general-purpose NLP model suitable for a wide range of language understanding and generation applications.\\ \hline
\texttt{yi:9b} & 5.0 & A large-scale language model designed for comprehensive understanding and generation capabilities.\\ \hline
\texttt{qwen2.5} & 4.7 & A language model series by Alibaba, pretrained on large-scale datasets, supporting extended context lengths.\\ \hline
\texttt{opencoder} & 4.7 & An encoder model optimized for processing and understanding input data in various NLP tasks.\\ \hline
\texttt{llama3.1} & 4.7 & A versatile model for natural language processing tasks, including text generation and summarization.\\ \hline
\texttt{zephyr} & 4.1 & A fine-tuned Mistral model for assistant-like tasks, available in various parameter sizes.\\ \hline
\texttt{neural-chat} & 4.1 & A conversational AI model designed for generating human-like dialogue responses.\\ \hline
\texttt{mistral} & 4.1 & A language model known for its balance between performance and efficiency in various NLP tasks.\\ \hline
\texttt{dolphin-mistral} & 4.1 & A variant of the Mistral model, fine-tuned for specialized language processing tasks.\\ \hline
\texttt{wizardlm2} & 4.1 & A language model tailored for advanced natural language understanding and generation.\\ \hline
\texttt{vicuna} & 3.8 & A general-use chat model based on Llama and Llama 2, optimized for conversational applications.\\ \hline
\texttt{nemotron-mini} & 2.7 & A compact model engineered for specific NLP applications requiring lower computational resources.\\ \hline
\texttt{phi3.5} & 2.2 & A language model designed for efficient natural language understanding and generation.\\ \hline
\texttt{granite3-moe} & 2.1 & A mixture of experts model aimed at enhancing grammatical accuracy in text processing.\\ \hline
\texttt{llama3.2} & 2.0 & A compact version of the Llama series, suitable for tasks requiring lower computational resources.\\ \hline
\texttt{granite3-dense} & 1.6 & A model focused on creating dense textual representations for improved semantic understanding.\\ \hline
\texttt{smollm2} & 1.8 & A compact language model tailored for efficient performance in text analysis and generation tasks.\\ \hline
\end{tabular}
\end{table}

\begin{figure*}[h!]
  \centering
  \includegraphics[width=\textwidth]{methods/Figure_1.png}
  \Description{A bar chart comparing the average response times of different NLP models, measured in milliseconds.
  Models with faster response times are better suited for real-time applications.}
  \caption[Average Response Time per Model]{A bar chart comparing the average response times of different NLP models, highlighting their suitability for real-time applications.
  Models such as \texttt{gpt-4o-mini} demonstrated the fastest response times, while others, such as \texttt{o1-preview}, showed significantly slower responses.}
  \label{fig:avg_response_time}
\end{figure*}

\begin{figure*}[h!]
  \centering
  \includegraphics[width=\textwidth]{methods/Figure_2.png}
  \Description{A bar chart showing the standard deviation of response times for each NLP model.
  Lower standard deviations indicate more stable response times.}
  \caption[Response Time Stability]{The stability of response times across different NLP models, measured by the standard deviation.
  Models like \texttt{gpt-4o-mini} exhibited high stability, whereas \texttt{o1-preview} displayed significant variability in its response times.}
  \label{fig:response_stability}
\end{figure*}

\begin{figure*}[h!]
  \centering
  \includegraphics[width=\textwidth]{methods/Figure_3.png}
  \Description{A grouped bar chart comparing the false positive and false negative rates of NLP models.
  Models with lower rates are more accurate in identifying grammatical errors.}
  \caption[False Positive and Negative Rates]{False positive and false negative rates for each NLP model, illustrating the models' accuracy in detecting grammatical errors.
  Models like \texttt{granite3-moe} achieved lower rates, indicating higher precision, while others exhibited higher error rates.}
  \label{fig:false_rates}
\end{figure*}

\begin{figure*}[h!]
  \centering
  \includegraphics[width=\textwidth]{methods/Figure_4.png}
  \Description{A bar chart presenting the accuracy of different NLP models in detecting grammatical errors, measured as a percentage.}
  \caption[Accuracy per Model]{Accuracy of NLP models in detecting grammatical errors.
  Higher accuracy was observed in models such as \texttt{gpt-4o-mini} and \texttt{phi3.5}, while others like \texttt{aya-expanse} showed lower performance in this metric.}
  \label{fig:accuracy}
\end{figure*}

\begin{figure*}[h!]
  \centering
  \includegraphics[width=\textwidth]{methods/Figure_5.png}
  \Description{A line chart showing the 25th, 50th (median), and 75th percentiles of response times for each NLP model.}
  \caption[Response Time Percentiles]{Percentiles of response times for NLP models, showcasing the 25th, 50th (median), and 75th percentiles.
  This provides insights into the consistency of response times, with models like \texttt{gpt-4o-mini} demonstrating more predictable performance compared to models such as \texttt{o1-preview}.}
  \label{fig:percentiles}
\end{figure*}

\subsection{Limitations and Future Directions}

\subsubsection{Current Limitations}
Despite its robust architecture and functional capabilities, the Dynawrite system has several limitations that constrain its scalability, performance, and comprehensiveness:
\begin{enumerate}
    \item \textbf{Limited Coverage of NLP Models}: While Dynawrite supports a diverse set of NLP models (e.g., GPT-4o, Llama3.2, Vicuna, etc.), it does not encompass the entirety of available models.
    Numerous NLP models remain unexplored, including specialized models for specific tasks, low-resource languages, or domain-specific applications.
    Additionally, with the rapid evolution of NLP technologies, many promising models are expected to emerge in the future, which the current system does not account for.
    
    \item \textbf{Dependency on Hardware and Paid APIs}: The integration of some NLP models, such as those provided by OpenAI, relies on paid APIs, which may not be accessible to all users.
    Similarly, the deployment of local models like those in the Ollama framework requires high-performance hardware (e.g., GPUs or advanced processors), limiting accessibility for institutions or individuals with constrained resources.
    
    \item \textbf{Scalability for Large-Scale Deployment}: The system's architecture, while modular, requires additional infrastructure investments to scale for a large number of concurrent users.
    This includes setting up monitoring, load balancing, and optimized storage for handling extensive datasets.
    
    \item \textbf{Evaluation Metrics}: Although the system captures basic analytics, such as response times and error detection accuracy, it lacks more nuanced evaluation metrics.
    For example, it does not analyze the linguistic complexity of hints or the cognitive impact of feedback on students.
    
    \item \textbf{User Experience}: While the system has been tested for functionality, there has been limited focus on conducting UX research to optimize the interface design and user interaction flow, especially for non-technical users.
\end{enumerate}

\subsubsection{Future Directions}
To address the identified limitations and enhance the overall utility of Dynawrite, the following directions are proposed for future development:
\begin{enumerate}
    \item \textbf{Expanding NLP Model Coverage}: Future iterations of Dynawrite will aim to integrate a broader range of NLP models, including:
    \begin{itemize}
        \item Domain-specific models for specialized tasks (e.g., legal, medical, or scientific texts).
        \item Low-resource language models to support underrepresented languages.
        \item Emerging state-of-the-art models that improve upon existing benchmarks.
    \end{itemize}
    The system will also include automated mechanisms for benchmarking and dynamically evaluating newly integrated models against existing ones.
    
    \item \textbf{Improved Accessibility and Offline Capabilities}: To reduce dependency on high-performance hardware and paid APIs, we aim to:
    \begin{itemize}
        \item Optimize local NLP model deployment for resource-constrained devices, such as mobile phones and edge devices.
        \item Develop offline-capable versions of Dynawrite, enabling users to access core functionalities without relying on an internet connection.
    \end{itemize}
    
    \item \textbf{Enhanced Scalability and Monitoring}: The system will be extended with tools for:
    \begin{itemize}
        \item Real-time performance monitoring and alerting to ensure uptime for large-scale deployments.
        \item Auto-scaling capabilities for handling varying workloads.
        \item Advanced data storage solutions to manage and process larger datasets efficiently.
    \end{itemize}
    
    \item \textbf{Refined Feedback Mechanisms}: Feedback generation will be enhanced by:
    \begin{itemize}
        \item Implementing adaptive feedback that adjusts to the skill level and learning pace of individual students.
        \item Providing multi-lingual support for error hints, catering to non-native English speakers.
        \item Incorporating cognitive theories into feedback design to maximize learning outcomes.
    \end{itemize}
    
    \item \textbf{Advanced Evaluation Metrics}: The system will include:
    \begin{itemize}
        \item Detailed analysis of linguistic complexity in feedback.
        \item Metrics assessing the pedagogical effectiveness of hints.
        \item Longitudinal tracking of user progress over time to evaluate learning improvements.
    \end{itemize}
    
    \item \textbf{User-Centric Design Enhancements}: Future iterations will prioritize UX research to:
    \begin{itemize}
        \item Simplify the interface for non-technical users.
        \item Introduce customization options for teachers and students, allowing personalized workflows.
        \item Add visual aids and interactive tutorials for new users.
    \end{itemize}
    
    \item \textbf{Collaboration with NLP Communities}: To keep pace with advancements in NLP, Dynawrite will engage with open-source and academic communities to:
    \begin{itemize}
        \item Incorporate cutting-edge models and tools as they are developed.
        \item Share anonymized usage data to contribute to the broader understanding of model performance in educational contexts.
    \end{itemize}
\end{enumerate}

\subsubsection{Anticipating Future NLP Developments}
Given the rapid pace of NLP advancements, Dynawrite acknowledges the potential emergence of groundbreaking technologies that may surpass current capabilities.
The system is designed to evolve alongside these developments, with an emphasis on:
\begin{itemize}
    \item Maintaining modularity for seamless integration of new models.
    \item Supporting experimentation with novel architectures, such as transformer-based or retrieval-augmented models.
    \item Leveraging innovations in explainable AI (XAI) to provide more transparent and interpretable feedback.
\end{itemize}

By addressing these limitations and embracing future directions, Dynawrite aims to remain at the forefront of NLP-based educational tools, offering robust functionality and adaptability to meet the needs of diverse user groups.
